On the Planning Abilities of Large Language Models : A Critical Investigation

Intrigued by the claims of emergent reasoning capabilities in LLMs trained on general web corpora, in this paper, we set out to investigate their planning capabilities. We aim to evaluate (1) the effectiveness of LLMs in generating plans autonomously in commonsense planning tasks and (2) the potential of LLMs in LLM-Modulo settings where they act as a source of heuristic guidance for external planners and verifiers. We conduct a systematic study by generating a suite of instances on domains similar to the ones employed in the International Planning Competition and evaluate LLMs in two distinct modes: autonomous and heuristic. Our findings reveal that LLMs' ability to generate executable plans autonomously is rather limited, with the best model (GPT-4) having an average success rate of ~12% across the domains. However, the results in the LLM-Modulo setting show more promise. In the LLM-Modulo setting, we demonstrate that LLM-generated plans can improve the search process for underlying sound planners and additionally show that external verifiers can help provide feedback on the generated plans and back-prompt the LLM for better plan generation.

==> human-in-the-loop.tex <==


\nsubsubsection{Human-in-the-loop mode}
Even though LLMs cannot provide sound plans by themselves, they may offer their insights as plan suggestions directly to the human-in-the-loop which might potentially guide the user
to the correct plan. After all, this sort of {\em computer supported cooperative work (CSCW)} use case has been the staple of LLM applications. 
%into a useful latent direction. 
We investigated the usefulness of LLMs for human planners by conducting a {\em between-subjects} user study. This user-study is similar in setup to the study described in section ~\ref{humanbaseline} with two key differences. (1) In this user study, there were two independent sets of participants. The first group of participants were not provided with any kind of assistance while coming up with plans (similar to the one in Section~\ref{humanbaseline}) whereas the other group were provided with an LLM generated suggestion that they could make use of. (2) At the end of the study, we have also asked both sets of participants to provide subjective feedback, using NASA-TLX \cite{hart1988development} assessment tool, to measure their cognitive load. 
%We utilized the NASA-TLX assessment tool to get feedback and measure the cognitive load of the users. 
Additionally, each participant in the second group had to provide feedback on whether the LLM-generated suggestion was correct when they were presented with the suggestion. We utilized the plans generated by GPT-4 to provide plan suggestions.
%
%
\karthik{We had 49 participants in the first group, where no assistance was provided, and 48 participants in the second group, where the LLM's plan was provided as a suggestion. We evaluated the statistical significance for the accuracy, time-taken and the cognitive load between the groups. Our findings revealed that the statistical signficance was not high.
\footnote{We performed independent-samples t-tests on the accuracy of the plans, the time taken to come up with a plan and the cognitive load of the task between the two groups. We set the significance level at $\alpha$=0.05 for the t-tests and ran them to see if the corresponding aspects between the LLM-assisted group and the group without LLM assistance are unequal. We received a statistic value of -1.21, 0.09 and -0.63, and a p-value of 0.22, 0.92 and 0.52 for the t-tests on accuracy, time taken and cognitive load respectively. This shows that we can't reject the null hypothesis for any of the tests and thus the difference in the accuracy, time-taken and cognitive load between the two groups is not statistically significant.} Further, 3 out of the 48 participants thought that the LLM suggestion was correct (when it was wrong) and 2 of them submitted the suggestion itself as the plan. This potentially hints at how these methods could feed into automation bias \cite{cummings2017automation}. Overall, the results showcase that there is no statistically significant difference between the two groups in terms of the accuracy, time taken and the cognitive load on the human planner.}







==> prompt_examples/blocksworld/back_prompt.tex <==
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.
Once you stack a block on top of a second block, the second block is no longer clear.

[STATEMENT]
As initial conditions I have that, the blue block is clear, the hand is empty, the blue block is on top of the orange block, the orange block is on top of the yellow block, the yellow block is on top of the red block and the red block is on the table.
My goal is to have that the red block is on top of the orange block and the yellow block is on top of the red block.

My plan is as follows:

[PLAN]
unstack the blue block from on top of the orange block
put down the blue block
unstack the orange block from on top of the yellow block
put down the orange block
unstack the yellow block from on top of the red block
stack the yellow block on top of the blue block
pick up the red block
stack the red block on top of the orange block
unstack the yellow block from on top of the blue block
stack the yellow block on top of the red block
[PLAN END]

[STATEMENT]
As initial conditions I have that, the yellow block is clear, the hand is empty, the red block is on top of the orange block, the orange block is on top of the blue block, the yellow block is on top of the red block and the blue block is on the table.
My goal is to have that the red block is on top of the yellow block and the yellow block is on top of the blue block.

My plan is as follows:

[PLAN]
--------------GPT-4 Response-----------------
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
stack the orange block on top of the red block
unstack the yellow block from on top of the red block
stack the yellow block on top of the blue block
pick up the red block
stack the red block on top of the yellow block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 1 has an unmet precondition:
unstack the red block from on top of the orange block
The unmet precondition is:
the red block is clear
--------------GPT-4 Response-----------------
Apologies for the mistake. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
stack the orange block on top of the red block
pick up the red block
stack the red block on top of the yellow block
pick up the yellow block
stack the yellow block on top of the blue block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 7 has an unmet precondition:
pick up the red block
The unmet precondition is:
the red block is clear
--------------GPT-4 Response-----------------
Apologies for the mistake again. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
stack the orange block on top of the red block
unstack the red block from on top of the orange block
stack the red block on top of the yellow block
pick up the yellow block
stack the yellow block on top of the blue block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid. The following action at step 7 has unmet preconditions:
unstack the red block from on top of the orange block
The unmet preconditions are:
the red block is clear and the red block is on top of the orange block
--------------GPT-4 Response-----------------
I apologize for the confusion. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
put down the orange block
pick up the red block
stack the red block on top of the yellow block
pick up the yellow block
stack the yellow block on top of the blue block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 9 has an unmet precondition:
pick up the yellow block
The unmet precondition is:
the yellow block is clear
--------------GPT-4 Response-----------------
I apologize for the mistakes in my previous plans. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
put down the orange block
pick up the blue block
stack the blue block on top of the yellow block
pick up the yellow block
stack the yellow block on top of the red block
pick up the red block
stack the red block on top of the orange block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 9 has an unmet precondition:
pick up the yellow block
The unmet precondition is:
the yellow block is clear
--------------GPT-4 Response-----------------
I apologize for the repeated mistakes. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
put down the orange block
pick up the red block
stack the red block on top of the yellow block
pick up the yellow block
stack the yellow block on top of the blue block
pick up the blue block
stack the blue block on top of the orange block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 9 has an unmet precondition:
pick up the yellow block
The unmet precondition is:
the yellow block is clear
--------------GPT-4 Response-----------------
I apologize for the confusion. Here's the corrected plan:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
put down the orange block
pick up the red block
stack the red block on top of the orange block
pick up the yellow block
stack the yellow block on top of the red block
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid. These are the unmet goal conditions:
the red block is on top of the yellow block and the yellow block is on top of the blue block
--------------GPT-4 Response-----------------
I apologize for the confusion in my previous plans. Here's the corrected plan to achieve the goal:

[PLAN]
unstack the yellow block from on top of the red block
put down the yellow block
unstack the red block from on top of the orange block
put down the red block
unstack the orange block from on top of the blue block
put down the orange block
pick up the yellow block
stack the yellow block on top of the blue block
pick up the red block
stack the red block on top of the yellow block
[PLAN END]
================SUCCESS================

==> prompt_examples/blocksworld/nl/domain.tex <==
========================================
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.
Once you stack a block on top of a second block, the second block is no longer clear. 
========================================

==> prompt_examples/blocksworld/nl/one-shot.tex <==
[STATEMENT]
As initial conditions I have that, the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table.
My goal is to have that the orange block is on top of the blue block.

My plan is as follows:

[PLAN]
unstack the blue block from on top of the orange block
put down the blue block
pick up the orange block
stack the orange block on top of the blue block
[PLAN END]

[STATEMENT]
As initial conditions I have that, the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table and the orange block is on the table.
My goal is to have that the orange block is on top of the red block.

My plan is as follows:

[PLAN]
--------- GPT-4 response ---------
unstack the yellow block from on top of the orange block
put down the yellow block
unstack the red block from on top of the blue block
put down the red block
pick up the orange block
stack the orange block on top of the red block
[PLAN END]
--------- Extracted plan ---------
(unstack yellow orange)
(put-down yellow)
(unstack red blue)
(put-down red)
(pick-up orange)
(stack orange red)

-------- Ground truth plan ---------
(unstack yellow orange)
(put-down yellow)
(pick-up orange)
(stack orange red)
================SUCCESS================

==> prompt_examples/blocksworld/nl/state-tracking.tex <==
The plan correctness is defined in terms of states resulting from executing the actions in the plan. An action is executable in a state when all its preconditions hold in that state. The state resulting from the action execution consists of everything in the previous state with the addition and deletion of add and delete effects of the action. Plan correctness is defined as follows: if the first action in the plan is applicable in the initial state, i.e., its preconditions are all present there; and the second action is applicable in the state resulting from applying the first action to the initial state, this process continues until the state resulting from the application of the last action in the last but one state gives rise to the final state where all the goals are satisfied.

[STATEMENT]
As initial conditions I have that, the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table
My goal is to have that the orange block is on top of the blue block.
My plan is as follows:

[PLAN]
1. Current State: the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table
   Action: unstack the blue block from on top of the orange block
   Reason: The above action is applicable in the current state because its preconditions; the blue block is clear, the hand is empty and the blue block is on top of the orange block, are satisfied in the current state.
   Resulting State: the red block is clear, the orange block is clear, the yellow block is clear, the hand is currently holding blue block, the red block is on the table, the orange block is on the table and the yellow block is on the table

2. Current State: the red block is clear, the orange block is clear, the yellow block is clear, the hand is currently holding blue block, the red block is on the table, the orange block is on the table and the yellow block is on the table
   Action: put down the blue block
   Reason: The above action is applicable in the current state because its preconditions; the hand is currently holding blue block, are satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the blue block is on the table, the orange block is on the table and the yellow block is on the table

3. Current State: the red block is clear, the blue block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the blue block is on the table, the orange block is on the table and the yellow block is on the table
   Action: pick up the orange block
   Reason: The above action is applicable in the current state because its preconditions; the orange block is clear, the hand is empty and the orange block is on the table, are satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the yellow block is clear, the hand is currently holding orange block, the red block is on the table, the blue block is on the table and the yellow block is on the table

4. Current State: the red block is clear, the blue block is clear, the yellow block is clear, the hand is currently holding orange block, the red block is on the table, the blue block is on the table and the yellow block is on the table
   Action: stack the orange block on top of the blue block
   Reason: The above action is applicable in the current state because its preconditions; the blue block is clear and the hand is currently holding orange block, are satisfied in the current state.
   Resulting State: the red block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the orange block is on top of the blue block, the red block is on the table, the blue block is on the table and the yellow block is on the table

Final State: the red block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the orange block is on top of the blue block, the red block is on the table, the blue block is on the table and the yellow block is on the table
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]

[STATEMENT]
As initial conditions I have that, the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table and the orange block is on the table
My goal is to have that the orange block is on top of the red block.
My plan is as follows:

[PLAN]

--------- GPT-4 response ---------
1. Current State: the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table, and the orange block is on the table
   Action: unstack the red block from on top of the blue block
   Reason: The above action is applicable in the current state because its preconditions; the red block is clear, the hand is empty, and the red block is on top of the blue block, are satisfied in the current state.
   Resulting State: the blue block is clear, the yellow block is clear, the hand is currently holding red block, the yellow block is on top of the orange block, the blue block is on the table, and the orange block is on the table

2. Current State: the blue block is clear, the yellow block is clear, the hand is currently holding red block, the yellow block is on top of the orange block, the blue block is on the table, and the orange block is on the table
   Action: put down the red block
   Reason: The above action is applicable in the current state because the precondition; the hand is currently holding red block, is satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the yellow block is on top of the orange block, the blue block is on the table, and the orange block is on the table

3. Current State: the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the yellow block is on top of the orange block, the blue block is on the table, and the orange block is on the table
   Action: unstack the yellow block from on top of the orange block
   Reason: The above action is applicable in the current state because its preconditions; the yellow block is clear, the hand is empty, and the yellow block is on top of the orange block, are satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the orange block is clear, the hand is currently holding yellow block, the red block is on the table, the blue block is on the table, and the orange block is on the table

4. Current State: the red block is clear, the blue block is clear, the orange block is clear, the hand is currently holding yellow block, the red block is on the table, the blue block is on the table, and the orange block is on the table
   Action: put down the yellow block
   Reason: The above action is applicable in the current state because the precondition; the hand is currently holding yellow block, is satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the blue block is on the table, the orange block is on the table, and the yellow block is on the table

5. Current State: the red block is clear, the blue block is clear, the orange block is clear, the yellow block is clear, the hand is empty, the red block is on the table, the blue block is on the table, the orange block is on the table, and the yellow block is on the table
   Action: pick up the orange block
   Reason: The above action is applicable in the current state because its preconditions; the orange block is clear, the hand is empty, and the orange block is on the table, are satisfied in the current state.
   Resulting State: the red block is clear, the blue block is clear, the hand is currently holding orange block, the yellow block is clear, the red block is on the table, the blue block is on the table, and the yellow block is on the table

6. Current State: the red block is clear, the blue block is clear, the hand is currently holding orange block, the yellow block is clear, the red block is on the table, the blue block is on the table, and the yellow block is on the table
   Action: stack the orange block on top of the red block
   Reason: The above action is applicable in the current state because its preconditions; the red block is clear, and the hand is currently holding orange block, are satisfied in the current state.
   Resulting State: the blue block is clear, the orange block is clear, the hand is empty, the yellow block is clear, the orange block is on top of the red block, the blue block is on the table, the red block is on the table, and the yellow block is on the table

Final State: the blue block is clear, the orange block is clear, the hand is empty, the yellow block is clear, the orange block is on top of the red block, the blue block is on the table, the red block is on the table, and the yellow block is on the table
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]
--------- Extracted plan ---------
(unstack red blue)
(put-down red)
(unstack yellow orange)
(put-down yellow)
(pick-up orange)
(stack orange red)
-------- Ground truth plan ---------
(unstack yellow orange)
(put-down yellow)
(pick-up orange)
(stack orange red)
================SUCCESS================

==> prompt_examples/blocksworld/nl/zero-shot.tex <==
[STATEMENT]
As initial conditions I have that, the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table.
My goal is to have that the orange block is on top of the blue block.

What is the plan to achieve my goal? Just give the actions in the plan.
--------- GPT-4 response ---------
1. Unstack the blue block from on top of the orange block
2. Put down the blue block on the table
3. Pick up the orange block
4. Stack the orange block on top of the blue block
--------- Extracted plan ---------
(unstack blue orange)
(put-down blue)
(pick-up orange)
(stack orange blue)

-------- Ground truth plan ---------
(unstack blue orange)
(put-down blue)
(pick-up orange)
(stack orange blue)
================SUCCESS================

==> prompt_examples/blocksworld/pddl/domain.tex <==
Here is a pddl domain, an example problem and it's corresponding plan. Provide the plan for the query problem. Provide only the pddl syntax for the plan.
[DOMAIN]
(define (domain blocksworld-4ops)
  (:requirements :strips)
(:predicates (clear ?x)
             (ontable ?x)
             (handempty)
             (holding ?x)
             (on ?x ?y))

(:action pick-up
  :parameters (?ob)
  :precondition (and (clear ?ob) (ontable ?ob) (handempty))
  :effect (and (holding ?ob) (not (clear ?ob)) (not (ontable ?ob))
               (not (handempty))))

(:action put-down
  :parameters  (?ob)
  :precondition (holding ?ob)
  :effect (and (clear ?ob) (handempty) (ontable ?ob)
               (not (holding ?ob))))

(:action stack
  :parameters  (?ob ?underob)
  :precondition (and (clear ?underob) (holding ?ob))
  :effect (and (handempty) (clear ?ob) (on ?ob ?underob)
               (not (clear ?underob)) (not (holding ?ob))))

(:action unstack
  :parameters  (?ob ?underob)
  :precondition (and (on ?ob ?underob) (clear ?ob) (handempty))
  :effect (and (holding ?ob) (clear ?underob)
               (not (on ?ob ?underob)) (not (clear ?ob)) (not (handempty)))))

==> prompt_examples/blocksworld/pddl/one-shot.tex <==
[PROBLEM]
(define (problem BW-rand-4)
(:domain blocksworld-4ops)
(:objects a b c d )
(:init
(handempty)
(ontable a)
(on b c)
(ontable c)
(ontable d)
(clear a)
(clear b)
(clear d)
)
(:goal
(and
(on c b))
)
)

[PLAN]
(unstack b c)
(put-down b)
(pick-up c)
(stack c b)
[PLAN_END]

[QUERY PROBLEM]
(define (problem BW-rand-4)
(:domain blocksworld-4ops)
(:objects a b c d )
(:init
(handempty)
(on a b)
(ontable b)
(ontable c)
(on d c)
(clear a)
(clear d)
)
(:goal
(and
(on c a))
)
)


--------- GPT-4 response ---------
[PLAN]
(unstack a b)
(put-down a)
(pick-up c)
(stack c a)
[PLAN_END]
--------- Extracted plan ---------
(unstack a b)
(put-down a)
(pick-up c)
(stack c a)
-------- Ground truth plan ---------
(unstack d c)
(put-down d)
(pick-up c)
(stack c a)
================FAILURE================

==> prompt_examples/blocksworld/pddl/zero-shot.tex <==
Here is a pddl domain, a planning problem. Provide the plan for the query problem. Provide only the pddl syntax for the plan where each action is represented as (ACTION_NAME OBJECTS).
[DOMAIN]
...
[QUERY PROBLEM]
(define (problem BW-rand-4)
(:domain blocksworld-4ops)
(:objects a b c d )
(:init
(handempty)
(ontable a)
(on b c)
(ontable c)
(ontable d)
(clear a)
(clear b)
(clear d)
)
(:goal
(and
(on c b))
)
)


--------- GPT-4 response ---------
Here is the plan for the query problem:

1. (unstack b c)
2. (put-down b)
3. (pick-up c)
4. (stack c b)
--------- Extracted plan ---------
(unstack b c)
(put-down b)
(pick-up c)
(stack c b)
-------- Ground truth plan ---------
(unstack b c)
(put-down b)
(pick-up c)
(stack c b)
================SUCCESS================

==> prompt_examples/logistics/back_prompt.tex <==
I have to plan logistics to transport packages within cities via trucks and between cities via airplanes. Locations within a city are directly connected (trucks can move between any two such locations), and so are the cities. In each city there is exactly one truck and each city has one location that serves as an airport.
Here are the actions that can be performed:

Load a package into a truck. For example, load package_1 into truck_1 at location_1_1.
Load a package into an airplane. For example, load package_1 into airplane_1 at location_1_1.
Unload a package from a truck. For example, unload package_1 from truck_1 at location_1_1.
Unload a package from an airplane. For example, unload package_1 from airplane_1 at location_1_1.
Drive a truck from one location to another location. For example, drive truck_1 from location_1_1 to location_1_2 in city_1.
Fly an airplane from one city to another city. For example, fly airplane_1 from location_1_1 to location_2_1. Here location_1_1 is the airport in city_1 and location_2_1 is the airport in city_2.

The following are the restrictions on the actions:
A package can be loaded into a truck only if the package and the truck are in the same location.
Once a package is loaded into a truck, the package is not at the location and is in the truck.   
A package can be loaded into an airplane only if the package and the airplane are in the same location.
Once a package is loaded into an airplane, the package is not at the location and is in the airplane.
A package can be unloaded from a truck only if the package is in the truck.
Once a package is unloaded from a truck, the package is not in the truck and is at the location of the truck.
A package can be unloaded from an airplane only if the package in the airplane.
Once a package is unloaded from an airplane, the package is not in the airplane and is at the location of the airplane.   
A truck can be driven from one location to another if the truck is at the from-location and both from-location and to-location are locations in the same city.
Once a truck is driven from one location to another, it is not at the from-location and is at the to-location.
An airplane can be flown from one city to another if the from-location and the to-location are airports and the airplane is at the from-location.
Once an airplane is flown from one city to another the airplane is not at the from-location and is at the to-location.

[STATEMENT]
As initial conditions I have that, location_0_0 is an airport, location_1_0 is an airport, airplane_0 is at location_1_0, package_0 is at location_1_0, package_1 is at location_0_0, truck_0 is at location_0_0, truck_1 is at location_1_0, location_0_0 is in the city city_0 and location_1_0 is in the city city_1.
My goal is to have that package_0 is at location_1_0 and package_1 is at location_1_0.

My plan is as follows:

[PLAN]
fly airplane_0 from location_1_0 to location_0_0
load package_1 into airplane_0 at location_0_0
fly airplane_0 from location_0_0 to location_1_0
unload package_1 from airplane_0 at location_1_0
[PLAN END]

[STATEMENT]
As initial conditions I have that, location_0_0 is an airport, location_1_0 is an airport, airplane_0 is at location_1_0, package_0 is at location_1_0, package_1 is at location_1_0, truck_0 is at location_0_0, truck_1 is at location_1_0, location_0_0 is in the city city_0 and location_1_0 is in the city city_1.
My goal is to have that package_0 is at location_0_0 and package_1 is at location_0_0.

My plan is as follows:

[PLAN]
--------------GPT-4 Response-----------------
fly airplane_0 from location_1_0 to location_0_0
load package_0 into airplane_0 at location_0_0
load package_1 into airplane_0 at location_0_0
fly airplane_0 from location_0_0 to location_1_0
unload package_0 from airplane_0 at location_1_0
unload package_1 from airplane_0 at location_1_0
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 2 has an unmet precondition:
load package_0 into airplane_0 at location_0_0
The unmet precondition is:
package_0 is at location_0_0
--------------GPT-4 Response-----------------
Apologies for the mistake. Here's the corrected plan:

[PLAN]
fly airplane_0 from location_1_0 to location_0_0
load package_0 into airplane_0 at location_1_0
load package_1 into airplane_0 at location_1_0
fly airplane_0 from location_0_0 to location_1_0
unload package_0 from airplane_0 at location_0_0
unload package_1 from airplane_0 at location_0_0
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 2 has an unmet precondition:
load package_0 into airplane_0 at location_1_0
The unmet precondition is:
airplane_0 is at location_1_0
--------------GPT-4 Response-----------------
I apologize for the mistake again. Here's the corrected plan:

[PLAN]
fly airplane_0 from location_1_0 to location_0_0
load package_0 into airplane_0 at location_0_0
load package_1 into airplane_0 at location_0_0
fly airplane_0 from location_0_0 to location_1_0
unload package_0 from airplane_0 at location_1_0
unload package_1 from airplane_0 at location_1_0
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 2 has an unmet precondition:
load package_0 into airplane_0 at location_0_0
The unmet precondition is:
package_0 is at location_0_0
--------------GPT-4 Response-----------------
I apologize for the confusion. Here's the corrected plan:

[PLAN]
fly airplane_0 from location_1_0 to location_0_0
load package_1 into airplane_0 at location_0_0
fly airplane_0 from location_0_0 to location_1_0
unload package_1 from airplane_0 at location_1_0
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 2 has an unmet precondition:
load package_1 into airplane_0 at location_0_0
The unmet precondition is:
package_1 is at location_0_0
--------------GPT-4 Response-----------------
I apologize for the repeated mistakes. Here's the corrected plan:

[PLAN]
fly airplane_0 from location_1_0 to location_0_0
load package_1 into airplane_0 at location_1_0
fly airplane_0 from location_0_0 to location_1_0
unload package_1 from airplane_0 at location_0_0
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 2 has an unmet precondition:
load package_1 into airplane_0 at location_1_0
The unmet precondition is:
airplane_0 is at location_1_0
--------------GPT-4 Response-----------------
I apologize once again for the mistakes. Here's the corrected plan:

[PLAN]
load package_0 into airplane_0 at location_1_0
load package_1 into airplane_0 at location_1_0
fly airplane_0 from location_1_0 to location_0_0
unload package_0 from airplane_0 at location_0_0
unload package_1 from airplane_0 at location_0_0
[PLAN END]
================SUCCESS================

==> prompt_examples/logistics/nl/domain.tex <==
I have to plan logistics to transport packages within cities via trucks and between cities via airplanes. Locations within a city are directly connected (trucks can move between any two such locations), and so are the cities. In each city there is exactly one truck and each city has one location that serves as an airport.
Here are the actions that can be performed:

Load a package into a truck.
Load a package into an airplane.
Unload a package from a truck.
Unload a package from an airplane.
Drive a truck from one location to another location.
Fly an airplane from one city to another city.

The following are the restrictions on the actions:
A package can be loaded into a truck only if the package and the truck are in the same location.
Once a package is loaded into a truck, the package is not at the location and is in the truck.   
A package can be loaded into an airplane only if the package and the airplane are in the same location.
Once a package is loaded into an airplane, the package is not at the location and is in the airplane.
A package can be unloaded from a truck only if the package is in the truck.
Once a package is unloaded from a truck, the package is not in the truck and is at the location of the truck.
A package can be unloaded from an airplane only if the package in the airplane.
Once a package is unloaded from an airplane, the package is not in the airplane and is at the location of the airplane.   
A truck can be driven from one location to another if the truck is at the from-location and both from-location and to-location are locations in the same city.
Once a truck is driven from one location to another, it is not at the from-location and is at the to-location.
An airplane can be flown from one city to another if the from-location and the to-location are airports and the airplane is at the from-location.
Once an airplane is flown from one city to another the airplane is not at the from-location and is at the to-location.

==> prompt_examples/logistics/nl/one-shot.tex <==
[STATEMENT]
As initial conditions I have that, location_0_0 is an airport, location_1_0 is an airport, airplane_0 is at location_0_0, airplane_1 is at location_0_0, package_0 is at location_1_0, truck_0 is at location_0_0, truck_1 is at location_1_0, location_0_0 is in the city city_0 and location_1_0 is in the city city_1.
My goal is to have that package_0 is at location_0_0.

My plan is as follows:

[PLAN]
fly airplane_1 from location_0_0 to location_1_0
load package_0 into airplane_1 at location_1_0
fly airplane_1 from location_1_0 to location_0_0
unload package_0 from airplane_1 at location_0_0
[PLAN END]

[STATEMENT]
As initial conditions I have that, location_0_0 is an airport, location_1_0 is an airport, airplane_0 is at location_1_0, airplane_1 is at location_1_0, package_0 is at location_1_0, truck_0 is at location_0_0, truck_1 is at location_1_0, location_0_0 is in the city city_0 and location_1_0 is in the city city_1.
My goal is to have that package_0 is at location_0_0.

My plan is as follows:

[PLAN]
--------- GPT-4 response ---------
load package_0 into airplane_1 at location_1_0
fly airplane_1 from location_1_0 to location_0_0
unload package_0 from airplane_1 at location_0_0
[PLAN END]
--------- Extracted plan ---------
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)

-------- Ground truth plan ---------
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)
================SUCCESS================

==> prompt_examples/logistics/nl/zero-shot.tex <==
I have to plan logistics to transport packages within cities via trucks and between cities via airplanes. Locations within a city are directly connected (trucks can move between any two such locations), and so are the cities. In each city there is exactly one truck and each city has one location that serves as an airport.
Here are the actions that can be performed:

Load a package into a truck. For example, load package_1 into truck_1 at location_1_1.
Load a package into an airplane. For example, load package_1 into airplane_1 at location_1_1.
Unload a package from a truck. For example, unload package_1 from truck_1 at location_1_1.
Unload a package from an airplane. For example, unload package_1 from airplane_1 at location_1_1.
Drive a truck from one location to another location. For example, drive truck_1 from location_1_1 to location_1_2 in city_1.
Fly an airplane from one city to another city. For example, fly airplane_1 from location_1_1 to location_2_1. Here location_1_1 is the airport in city_1 and location_2_1 is the airport in city_2.

The following are the restrictions on the actions:
A package can be loaded into a truck only if the package and the truck are in the same location.
Once a package is loaded into a truck, the package is not at the location and is in the truck.   
A package can be loaded into an airplane only if the package and the airplane are in the same location.
Once a package is loaded into an airplane, the package is not at the location and is in the airplane.
A package can be unloaded from a truck only if the package is in the truck.
Once a package is unloaded from a truck, the package is not in the truck and is at the location of the truck.
A package can be unloaded from an airplane only if the package in the airplane.
Once a package is unloaded from an airplane, the package is not in the airplane and is at the location of the airplane.   
A truck can be driven from one location to another if the truck is at the from-location and both from-location and to-location are locations in the same city.
Once a truck is driven from one location to another, it is not at the from-location and is at the to-location.
An airplane can be flown from one city to another if the from-location and the to-location are airports and the airplane is at the from-location.
Once an airplane is flown from one city to another the airplane is not at the from-location and is at the to-location.

[STATEMENT]
As initial conditions I have that, location_0_0 is an airport, location_1_0 is an airport, airplane_0 is at location_0_0, airplane_1 is at location_0_0, package_0 is at location_1_0, truck_0 is at location_0_0, truck_1 is at location_1_0, location_0_0 is in the city city_0 and location_1_0 is in the city city_1.
My goal is to have that package_0 is at location_0_0.

What is the plan to achieve my goal? Just give the actions in the plan.
--------- GPT-4 response ---------
1. Load package_0 into truck_1 at location_1_0.
2. Drive truck_1 from location_1_0 to location_0_0 in city_1.
3. Unload package_0 from truck_1 at location_0_0.
4. Load package_0 into airplane_1 at location_0_0.
5. Fly airplane_1 from location_0_0 to location_1_0.
6. Unload package_0 from airplane_1 at location_1_0.
7. Load package_0 into truck_0 at location_1_0.
8. Fly airplane_0 from location_0_0 to location_1_0.
9. Drive truck_0 from location_1_0 to location_0_0 in city_0.
10. Unload package_0 from truck_0 at location_0_0.
--------- Extracted plan ---------
(load-truck p0 t1 l1-0)
(drive-truck t1 l1-0 l0-0 c1)
(unload-truck p0 t1 l0-0)
(load-airplane p0 a1 l0-0)
(fly-airplane a1 l0-0 l1-0)
(unload-airplane p0 a1 l1-0)
(load-truck p0 t0 l1-0)
(fly-airplane a0 l0-0 l1-0)
(drive-truck t0 l1-0 l0-0 c0)
(unload-truck p0 t0 l0-0)

-------- Ground truth plan ---------
(fly-airplane a1 l0-0 l1-0)
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)
================FAILURE================

==> prompt_examples/logistics/pddl/domain.tex <==
Here is a pddl domain, an example problem and it's corresponding plan. Provide the plan for the query problem. Provide only the pddl syntax for the plan.
[DOMAIN]
(define (domain logistics-strips)
  (:requirements :strips) 
  (:predicates 	(OBJ ?obj)
	       	(TRUCK ?truck)
               	(LOCATION ?loc)
		(AIRPLANE ?airplane)
                (CITY ?city)
                (AIRPORT ?airport)
		(at ?obj ?loc)
		(in ?obj1 ?obj2)
		(in-city ?obj ?city))
 
  ; (:types )		; default object

(:action LOAD-TRUCK
  :parameters
   (?obj
    ?truck
    ?loc)
  :precondition
   (and (OBJ ?obj) (TRUCK ?truck) (LOCATION ?loc)
   (at ?truck ?loc) (at ?obj ?loc))
  :effect
   (and (not (at ?obj ?loc)) (in ?obj ?truck)))

(:action LOAD-AIRPLANE
  :parameters
   (?obj
    ?airplane
    ?loc)
  :precondition
   (and (OBJ ?obj) (AIRPLANE ?airplane) (LOCATION ?loc)
   (at ?obj ?loc) (at ?airplane ?loc))
  :effect
   (and (not (at ?obj ?loc)) (in ?obj ?airplane)))



(:action UNLOAD-TRUCK
  :parameters
   (?obj
    ?truck
    ?loc)
  :precondition
   (and (OBJ ?obj) (TRUCK ?truck) (LOCATION ?loc)
        (at ?truck ?loc) (in ?obj ?truck))
  :effect
   (and (not (in ?obj ?truck)) (at ?obj ?loc)))

(:action UNLOAD-AIRPLANE
  :parameters
   (?obj
    ?airplane
    ?loc)
  :precondition
   (and (OBJ ?obj) (AIRPLANE ?airplane) (LOCATION ?loc)
        (in ?obj ?airplane) (at ?airplane ?loc))
  :effect
   (and (not (in ?obj ?airplane)) (at ?obj ?loc)))

(:action DRIVE-TRUCK
  :parameters
   (?truck
    ?loc-from
    ?loc-to
    ?city)
  :precondition
   (and (TRUCK ?truck) (LOCATION ?loc-from) (LOCATION ?loc-to) (CITY ?city)
   (at ?truck ?loc-from)
   (in-city ?loc-from ?city)
   (in-city ?loc-to ?city))
  :effect
   (and (not (at ?truck ?loc-from)) (at ?truck ?loc-to)))

(:action FLY-AIRPLANE
  :parameters
   (?airplane
    ?loc-from
    ?loc-to)
  :precondition
   (and (AIRPLANE ?airplane) (AIRPORT ?loc-from) (AIRPORT ?loc-to)
	(at ?airplane ?loc-from))
  :effect
   (and (not (at ?airplane ?loc-from)) (at ?airplane ?loc-to)))
)

==> prompt_examples/logistics/pddl/one-shot.tex <==
[PROBLEM]
(define (problem logistics-c2-s1-p1-a2)
(:domain logistics-strips)
(:objects a0 a1 
          c0 c1 
          t0 t1 
          l0-0 l1-0 
          p0 
)
(:init
    (AIRPLANE a0)
    (AIRPLANE a1)
    (CITY c0)
    (CITY c1)
    (TRUCK t0)
    (TRUCK t1)
    (LOCATION l0-0)
    (in-city  l0-0 c0)
    (LOCATION l1-0)
    (in-city  l1-0 c1)
    (AIRPORT l0-0)
    (AIRPORT l1-0)
    (OBJ p0)
    (at t0 l0-0)
    (at t1 l1-0)
    (at p0 l1-0)
    (at a0 l0-0)
    (at a1 l0-0)
)
(:goal
    (and
        (at p0 l0-0)
    )
)
)

[PLAN]
(fly-airplane a1 l0-0 l1-0)
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)
[PLAN_END]

[QUERY PROBLEM]
(define (problem logistics-c2-s1-p1-a2)
(:domain logistics-strips)
(:objects a0 a1 
          c0 c1 
          t0 t1 
          l0-0 l1-0 
          p0 
)
(:init
    (AIRPLANE a0)
    (AIRPLANE a1)
    (CITY c0)
    (CITY c1)
    (TRUCK t0)
    (TRUCK t1)
    (LOCATION l0-0)
    (in-city  l0-0 c0)
    (LOCATION l1-0)
    (in-city  l1-0 c1)
    (AIRPORT l0-0)
    (AIRPORT l1-0)
    (OBJ p0)
    (at t0 l0-0)
    (at t1 l1-0)
    (at p0 l1-0)
    (at a0 l1-0)
    (at a1 l1-0)
)
(:goal
    (and
        (at p0 l0-0)
    )
)
)


--------- GPT-4 response ---------
Based on the provided domain, problem, and example plan, here is the PDDL syntax for the plan corresponding to the query problem:

(fly-airplane a0 l1-0 l0-0)
(load-airplane p0 a0 l1-0)
(fly-airplane a0 l0-0 l1-0)
(unload-airplane p0 a0 l1-0)
--------- Extracted plan ---------
(fly-airplane a0 l1-0 l0-0)
(load-airplane p0 a0 l1-0)
(fly-airplane a0 l0-0 l1-0)
(unload-airplane p0 a0 l1-0)
-------- Ground truth plan ---------
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)
================FAILURE================

==> prompt_examples/logistics/pddl/zero-shot.tex <==
Here is a pddl domain, a planning problem. Provide the plan for the query problem. Provide only the pddl syntax for the plan where each action is represented as (ACTION_NAME OBJECTS).
[DOMAIN]
...
[QUERY PROBLEM]
(define (problem logistics-c2-s1-p1-a2)
(:domain logistics-strips)
(:objects a0 a1 
          c0 c1 
          t0 t1 
          l0-0 l1-0 
          p0 
)
(:init
    (AIRPLANE a0)
    (AIRPLANE a1)
    (CITY c0)
    (CITY c1)
    (TRUCK t0)
    (TRUCK t1)
    (LOCATION l0-0)
    (in-city  l0-0 c0)
    (LOCATION l1-0)
    (in-city  l1-0 c1)
    (AIRPORT l0-0)
    (AIRPORT l1-0)
    (OBJ p0)
    (at t0 l0-0)
    (at t1 l1-0)
    (at p0 l1-0)
    (at a0 l0-0)
    (at a1 l0-0)
)
(:goal
    (and
        (at p0 l0-0)
    )
)
)


--------- GPT-4 response ---------
Based on the provided domain and problem, the plan to achieve the goal state could be:

1. LOAD-AIRPLANE p0 on a0 at l1-0
2. FLY-AIRPLANE a0 from l1-0 to l0-0
3. UNLOAD-AIRPLANE p0 from a0 at l0-0

Here is the PDDL syntax for the plan:

(LOAD-AIRPLANE p0 a0 l1-0)
(FLY-AIRPLANE a0 l1-0 l0-0)
(UNLOAD-AIRPLANE p0 a0 l0-0)
--------- Extracted plan ---------
(load-airplane p0 a0 l1-0)
(fly-airplane a0 l1-0 l0-0)
(unload-airplane p0 a0 l0-0)
-------- Ground truth plan ---------
(fly-airplane a1 l0-0 l1-0)
(load-airplane p0 a1 l1-0)
(fly-airplane a1 l1-0 l0-0)
(unload-airplane p0 a1 l0-0)
================FAILURE================

==> prompt_examples/mystery/back_prompt.tex <==
I am playing with a set of objects. Here are the actions I can do

   Attack object
   Feast object from another object
   Succumb object
   Overcome object from another object

I have the following restrictions on my actions:
    To perform Attack action, the following facts need to be true: Province object, Planet object, Harmony.
    Once Attack action is performed the following facts will be true: Pain object.
    Once Attack action is performed the following facts will be false: Province object, Planet object, Harmony.
    To perform Succumb action, the following facts need to be true: Pain object.
    Once Succumb action is performed the following facts will be true: Province object, Planet object, Harmony.    
    Once Succumb action is performed the following facts will be false: Pain object.
    To perform Overcome action, the following needs to be true: Province other object, Pain object.
    Once Overcome action is performed the following will be true: Harmony, Pain object, Object Craves other object.
    Once Overcome action is performed the following will be false: Province other object, Pain object.
    To perform Feast action, the following needs to be true: Object Craves other object, Province object, Harmony.
    Once Feast action is performed the following will be true: Pain object, Province other object.
    Once Feast action is performed the following will be false:, Object Craves other object, Province object, Harmony.

[STATEMENT]
As initial conditions I have that, object b craves object c, harmony, planet object a, planet object c, planet object d, province object a, province object b and province object d.
My goal is to have that object c craves object b.

My plan is as follows:

[PLAN]
feast object b from object c
succumb object b
attack object c
overcome object c from object b
[PLAN END]

[STATEMENT]
As initial conditions I have that, object a craves object b, object d craves object c, harmony, planet object b, planet object c, province object a and province object d.
My goal is to have that object c craves object a.

My plan is as follows:

[PLAN]
--------------GPT-4 Response-----------------
feast object a from object b
succumb object a
attack object d
overcome object d from object c
feast object c from object a
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 3 has an unmet precondition:
attack object d
The unmet precondition is:
planet object d
--------------GPT-4 Response-----------------
Apologies for the oversight. Here's the corrected plan:

[PLAN]
feast object a from object b
succumb object a
attack object c
overcome object c from object d
feast object d from object c
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 3 has an unmet precondition:
attack object c
The unmet precondition is:
province object c
--------------GPT-4 Response-----------------
I apologize for the mistake. Here's another attempt at a valid plan:

[PLAN]
feast object a from object b
succumb object a
attack object b
overcome object b from object c
feast object c from object d
succumb object c
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 4 has an unmet precondition:
overcome object b from object c
The unmet precondition is:
province object c
--------------GPT-4 Response-----------------
I apologize for the repeated mistakes. Here's a new plan:

[PLAN]
feast object a from object b
succumb object a
attack object b
overcome object b from object a
feast object a from object d
succumb object a
attack object d
overcome object d from object c
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid. The following action at step 5 has unmet preconditions:
feast object a from object d
The unmet preconditions are:
object a craves object d and province object a
--------------GPT-4 Response-----------------
I apologize for the errors in my previous plans. Here's a revised plan:

[PLAN]
feast object a from object b
succumb object a
attack object b
overcome object b from object a
attack object c
succumb object c
feast object c from object a
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 5 has an unmet precondition:
attack object c
The unmet precondition is:
province object c
--------------GPT-4 Response-----------------
I apologize for the continued mistakes. Here's another attempt at a valid plan:

[PLAN]
feast object a from object b
succumb object a
attack object b
overcome object b from object a
feast object d from object c
succumb object d
attack object c
overcome object c from object a
[PLAN END]
--------------VAL Feedback-----------------
The above plan is invalid.The following action at step 8 has an unmet precondition:
overcome object c from object a
The unmet precondition is:
province object a
--------------GPT-4 Response-----------------
I apologize for the errors in my previous plans. After reevaluating the problem, I have determined that it is not possible to achieve the goal of having object c crave object a given the initial conditions and action restrictions provided.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
--------------VAL Feedback-----------------
The above plan is invalid. This is the unmet goal condition:
object c craves object a
--------------GPT-4 Response-----------------
You are correct, the goal of having object c crave object a has not been met in the previous plans. Given the initial conditions and action restrictions provided, it appears that it is not possible to achieve this goal.
================FAILURE================

==> prompt_examples/mystery/nl/domain.tex <==
I am playing with a set of objects. Here are the actions I can do

   Attack object
   Feast object from another object
   Succumb object
   Overcome object from another object

I have the following restrictions on my actions:
    To perform Attack action, the following facts need to be true: Province object, Planet object, Harmony.
    Once Attack action is performed the following facts will be true: Pain object.
    Once Attack action is performed the following facts will be false: Province object, Planet object, Harmony.
    To perform Succumb action, the following facts need to be true: Pain object.
    Once Succumb action is performed the following facts will be true: Province object, Planet object, Harmony.    
    Once Succumb action is performed the following facts will be false: Pain object.
    To perform Overcome action, the following needs to be true: Province other object, Pain object.
    Once Overcome action is performed the following will be true: Harmony, Province object, Object Craves other object.
    Once Overcome action is performed the following will be false: Province other object, Pain object.
    To perform Feast action, the following needs to be true: Object Craves other object, Province object, Harmony.
    Once Feast action is performed the following will be true: Pain object, Province other object.
    Once Feast action is performed the following will be false:, Object Craves other object, Province object, Harmony.

==> prompt_examples/mystery/nl/one-shot.tex <==
[STATEMENT]
As initial conditions I have that, province object a, province object b, province object d, harmony, object b craves object c, planet object a, planet object c and planet object d.
My goal is to have that object c craves object b.

My plan is as follows:

[PLAN]
feast object b from object c
succumb object b
attack object c
overcome object c from object b
[PLAN END]

[STATEMENT]
As initial conditions I have that, province object a, province object d, harmony, object a craves object b, object d craves object c, planet object b and planet object c.
My goal is to have that object c craves object a.

My plan is as follows:

[PLAN]
--------- GPT-4 response ---------
feast object a from object b
succumb object a
attack object d
overcome object d from object a
feast object c from object a
[PLAN END]
--------- Extracted plan ---------
(feast a b)
(succumb a)
(attack d)
(overcome d a)
(feast c a)

-------- Ground truth plan ---------
(feast object d object c)
(succumb object d)
(attack object c)
(overcome object c object a)
================FAILURE================

==> prompt_examples/mystery/nl/state-tracking.tex <==
The plan correctness is defined in terms of states resulting from executing the actions in the plan. An action is executable in a state when all its preconditions hold in that state. The state resulting from the action execution consists of everything in the previous state with the addition and deletion of add and delete effects of the action. Plan correctness is defined as follows: if the first action in the plan is applicable in the initial state, i.e., its preconditions are all present there; and the second action is applicable in the state resulting from applying the first action to the initial state, this process continues until the state resulting from the application of the last action in the last but one state gives rise to the final state where all the goals are satisfied.

[STATEMENT]
As initial conditions I have that, object b craves object c, harmony, planet object a, planet object c, planet object d, province object a, province object b and province object d
My goal is to have that object c craves object b.
My plan is as follows:

[PLAN]
1. Current State: object b craves object c, harmony, planet object a, planet object c, planet object d, province object a, province object b and province object d
   Action: feast object b from object c
   Reason: The above action is applicable in the current state because its preconditions; object b craves object c, harmony and province object b, are satisfied in the current state.
   Resulting State: pain object b, planet object a, planet object c, planet object d, province object a, province object c and province object d

2. Current State: pain object b, planet object a, planet object c, planet object d, province object a, province object c and province object d
   Action: succumb object b
   Reason: The above action is applicable in the current state because its preconditions; pain object b, are satisfied in the current state.
   Resulting State: harmony, planet object a, planet object b, planet object c, planet object d, province object a, province object b, province object c and province object d

3. Current State: harmony, planet object a, planet object b, planet object c, planet object d, province object a, province object b, province object c and province object d
   Action: attack object c
   Reason: The above action is applicable in the current state because its preconditions; harmony, planet object c and province object c, are satisfied in the current state.
   Resulting State: pain object c, planet object a, planet object b, planet object d, province object a, province object b and province object d

4. Current State: pain object c, planet object a, planet object b, planet object d, province object a, province object b and province object d
   Action: overcome object c from object b
   Reason: The above action is applicable in the current state because its preconditions; pain object c and province object b, are satisfied in the current state.
   Resulting State: object c craves object b, harmony, planet object a, planet object b, planet object d, province object a, province object c and province object d

Final State: object c craves object b, harmony, planet object a, planet object b, planet object d, province object a, province object c and province object d
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]

[STATEMENT]
As initial conditions I have that, object a craves object b, object d craves object c, harmony, planet object b, planet object c, province object a and province object d
My goal is to have that object c craves object a.
My plan is as follows:

[PLAN]
--------- GPT-4 response ---------
1. Current State: object a craves object b, object d craves object c, harmony, planet object b, planet object c, province object a and province object d
   Action: attack object d
   Reason: The above action is applicable in the current state because its preconditions; planet object d, province object d, and harmony, are satisfied in the current state.
   Resulting State: pain object d, planet object b, planet object c, province object a, province object b, and province object c

2. Current State: pain object d, planet object b, planet object c, province object a, province object b, and province object c
   Action: overcome object d from object a
   Reason: The above action is applicable in the current state because its preconditions; pain object d and province object a, are satisfied in the current state.
   Resulting State: object d craves object a, harmony, planet object b, planet object c, province object a, province object b, province object c, and province object d

3. Current State: object a craves object b, object d craves object a, harmony, planet object b, planet object c, province object a, province object b, province object c, and province object d
   Action: attack object b
   Reason: The above action is applicable in the current state because its preconditions; harmony, planet object b, and province object b, are satisfied in the current state.
   Resulting State: pain object b, planet object c, province object a, province object c, and province object d
   
4. Current State: pain object b, planet object c, province object a, province object c, and province object d
   Action: succumb object b
   Reason: The above action is applicable in the current state because its preconditions; pain object b, are satisfied in the current state.
   Resulting State: harmony, planet object c, planet object b, province object a, province object b, province object c, and province object d

5. Current State: harmony, planet object c, planet object b, province object a, province object b, province object c and province object d
   Action: attack object c
   Reason: The above action is applicable in the current state because its preconditions; harmony, planet object c, province object c, are satisfied in the current state.
   Resulting State: pain object c, planet object b, province object a, province object b, and province object d

6. Current State: pain object c, planet object b, province object a, province object b, and province object d
   Action: overcome object c from object a
   Reason: The above action is applicable in the current state because its preconditions; pain object c and province object a, are satisfied in the current state.
   Resulting State: object c craves object a, harmony, planet object b, planet object d, province object a, province object b and province object d

Final State: object c craves object a, harmony, planet object b, planet object d, province object a, province object b and province object d
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]
--------- Extracted plan ---------
(attack object d)
(overcome object d object a)
(attack object b)
(succumb object b)
(attack object c)
(overcome object c object a)

-------- Ground truth plan ---------
(feast object d object c)
(succumb object d)
(attack object c)
(overcome object c object a)
================FAILURE================

==> prompt_examples/mystery/nl/zero-shot.tex <==
[STATEMENT]
As initial conditions I have that, object a craves object b, object d craves object c, harmony, planet object b, planet object c, province object a and province object d.
My goal is to have that object c craves object a.

What is the plan to achieve my goal? Just give the actions in the plan.
--------- GPT-4 response ---------
1. Feast object a from object b
2. Attack object a
3. Succumb object a
4. Overcome object a from object c
5. Feast object c from object a
--------- Extracted plan ---------
(feast a b)
(attack a)
(succumb a)
(overcome a c)
(feast c a)

-------- Ground truth plan ---------
(feast d c)
(succumb d)
(attack c)
(overcome c a)
================FAILURE================

==> prompt_examples/mystery/pddl/domain.tex <==
Here is a pddl domain, a planning problem. Provide the plan for the query problem. Provide only the pddl syntax.
[DOMAIN]
(define (domain mystery-4ops)
  (:requirements :strips)
(:predicates (province ?x)
             (planet ?x)
             (harmony)
             (pain ?x)
             (craves ?x ?y))

(:action attack
  :parameters (?ob)
  :precondition (and (province ?ob) (planet ?ob) (harmony))
  :effect (and (pain ?ob) (not (province ?ob)) (not (planet ?ob))
               (not (harmony))))

(:action succumb
  :parameters  (?ob)
  :precondition (pain ?ob)
  :effect (and (province ?ob) (harmony) (planet ?ob)
               (not (pain ?ob))))

(:action overcome
  :parameters  (?ob ?underob)
  :precondition (and (province ?underob) (pain ?ob))
  :effect (and (harmony) (province ?ob) (craves ?ob ?underob)
               (not (province ?underob)) (not (pain ?ob))))

(:action feast
  :parameters  (?ob ?underob)
  :precondition (and (craves ?ob ?underob) (province ?ob) (harmony))
  :effect (and (pain ?ob) (province ?underob)
               (not (craves ?ob ?underob)) (not (province ?ob)) (not (harmony)))))


==> prompt_examples/mystery/pddl/one-shot.tex <==
[PROBLEM]
(define (problem MY-rand-4)
(:domain mystery-4ops)
(:objects a b c d )
(:init
(harmony)
(planet a)
(craves b c)
(planet c)
(planet d)
(province a)
(province b)
(province d)
)
(:goal
(and
(craves c b))
)
)

[PLAN]
(feast b c)
(succumb b)
(attack c)
(overcome c b)
[PLAN_END]

[QUERY PROBLEM]
(define (problem MY-rand-4)
(:domain mystery-4ops)
(:objects a b c d )
(:init
(harmony)
(craves a b)
(planet b)
(planet c)
(craves d c)
(province a)
(province d)
)
(:goal
(and
(craves c a))
)
)


--------- GPT-4 response ---------
[QUERY_PLAN]
(feast a b)
(succumb a)
(attack c)
(overcome c a)
[QUERY_PLAN_END]
--------- Extracted plan ---------
(feast a b)
(succumb a)
(attack c)
(overcome c a)
-------- Ground truth plan ---------
(feast d c)
(succumb d)
(attack c)
(overcome c a)
================FAILURE================

==> prompt_examples/mystery/pddl/zero-shot.tex <==
Here is a pddl domain, a planning problem. Provide the plan for the query problem. Provide only the pddl syntax for the plan where each action is represented as (ACTION_NAME OBJECTS).
[DOMAIN]
...
[QUERY PROBLEM]
(define (problem MY-rand-4)
(:domain mystery-4ops)
(:objects a b c d )
(:init
(harmony)
(planet a)
(craves b c)
(planet c)
(planet d)
(province a)
(province b)
(province d)
)
(:goal
(and
(craves c b))
)
)


--------- GPT-4 response ---------
Here is the PDDL syntax for the plan:

1. (attack a)
2. (overcome b a)
3. (feast b d)
4. (succumb d)
5. (overcome c b)
--------- Extracted plan ---------
(attack a)
(overcome b a)
(feast b d)
(succumb d)
(overcome c b)
-------- Ground truth plan ---------
(feast b c)
(succumb b)
(attack c)
(overcome c b)
================FAILURE================

==> prompt_examples/mystery/randomized/domain.tex <==
I am playing with a set of objects. Here are the actions I can do

   1jpkithdyjmlikck object
   xptxjrdkbi3pqsqr object from another object
   9big8ruzarkkquyu object
   2ijg9q8swj2shjel object from another object

I have the following restrictions on my actions:
    To perform 1jpkithdyjmlikck action, the following facts need to be true: aqcjuuehivl8auwt object, 51nbwlachmfartjn object, 3covmuy4yrjthijd.
    Once 1jpkithdyjmlikck action is performed the following facts will be true: gk5asm3f7u1fekpj object.
    Once 1jpkithdyjmlikck action is performed the following facts will be false: aqcjuuehivl8auwt object, 51nbwlachmfartjn object, 3covmuy4yrjthijd.
    To perform 9big8ruzarkkquyu action, the following facts need to be true: gk5asm3f7u1fekpj object.
    Once 9big8ruzarkkquyu action is performed the following facts will be true: aqcjuuehivl8auwt object, 51nbwlachmfartjn object, 3covmuy4yrjthijd.    
    Once 9big8ruzarkkquyu action is performed the following facts will be false: gk5asm3f7u1fekpj object.
    To perform 2ijg9q8swj2shjel action, the following needs to be true: aqcjuuehivl8auwt other object, gk5asm3f7u1fekpj object.
    Once 2ijg9q8swj2shjel action is performed the following will be true: 3covmuy4yrjthijd, aqcjuuehivl8auwt object, Object 4DMF1cMTYXGSP94G other object.
    Once 2ijg9q8swj2shjel action is performed the following will be false: aqcjuuehivl8auwt other object, gk5asm3f7u1fekpj object.
    To perform xptxjrdkbi3pqsqr action, the following needs to be true: Object 4DMF1cMTYXGSP94G other object, aqcjuuehivl8auwt object, 3covmuy4yrjthijd.
    Once xptxjrdkbi3pqsqr action is performed the following will be true: gk5asm3f7u1fekpj object, aqcjuuehivl8auwt other object.
    Once xptxjrdkbi3pqsqr action is performed the following will be false:, Object 4DMF1cMTYXGSP94G other object, aqcjuuehivl8auwt object, 3covmuy4yrjthijd.


==> prompt_examples/mystery/randomized/one-shot.tex <==
[STATEMENT]
As initial conditions I have that, aqcjuuehivl8auwt object a, aqcjuuehivl8auwt object b, aqcjuuehivl8auwt object d, 3covmuy4yrjthijd, object b 4dmf1cmtyxgsp94g object c, 51nbwlachmfartjn object a, 51nbwlachmfartjn object c and 51nbwlachmfartjn object d.
My goal is to have that object c 4dmf1cmtyxgsp94g object b.

My plan is as follows:

[PLAN]
xptxjrdkbi3pqsqr object b from object c
9big8ruzarkkquyu object b
1jpkithdyjmlikck object c
2ijg9q8swj2shjel object c from object b
[PLAN END]

[STATEMENT]
As initial conditions I have that, aqcjuuehivl8auwt object a, aqcjuuehivl8auwt object d, 3covmuy4yrjthijd, object a 4dmf1cmtyxgsp94g object b, object d 4dmf1cmtyxgsp94g object c, 51nbwlachmfartjn object b and 51nbwlachmfartjn object c.
My goal is to have that object c 4dmf1cmtyxgsp94g object a.

My plan is as follows:

[PLAN]
--------- GPT-4 response ---------
xptxjrdkbi3pqsqr object a from object b
9big8ruzarkkquyu object a
1jpkithdyjmlikck object d
2ijg9q8swj2shjel object d from object c
[PLAN END]
--------- Extracted plan ---------
(xptxjrdkbi3pqsqr object a object b)
(9big8ruzarkkquyu object a)
(1jpkithdyjmlikck object d)
(2ijg9q8swj2shjel object d object c)

-------- Ground truth plan ---------
(xptxjrdkbi3pqsqr object d object c)
(9big8ruzarkkquyu object d)
(1jpkithdyjmlikck object c)
(2ijg9q8swj2shjel object c object a)
================FAILURE================

==> prompt_examples/mystery/randomized/zero-shot.tex <==
[STATEMENT]
As initial conditions I have that, aqcjuuehivl8auwt object a, aqcjuuehivl8auwt object b, aqcjuuehivl8auwt object d, 3covmuy4yrjthijd, object b 4dmf1cmtyxgsp94g object c, 51nbwlachmfartjn object a, 51nbwlachmfartjn object c and 51nbwlachmfartjn object d.
My goal is to have that object c 4dmf1cmtyxgsp94g object b.

What is the plan to achieve my goal? Just give the actions in the plan.
--------- GPT3 response ---------
1. 1jpkithdyjmlikck object A
2. 2ijg9q8swj2shjel object A from object B
3. xptxjrdkbi3pqsqr object C from object A
4. 9big8ruzarkkquyu object A
--------- Extracted plan ---------
(1jpkithdyjmlikck object a)
(2ijg9q8swj2shjel object a object b)
(xptxjrdkbi3pqsqr object c object a)
(9big8ruzarkkquyu object a)

-------- Ground truth plan ---------
(xptxjrdkbi3pqsqr object b object c)
(9big8ruzarkkquyu object b)
(1jpkithdyjmlikck object c)
(2ijg9q8swj2shjel object c object b)
================FAILURE================

==> prompt_examples/pddl_action_desc.tex <==
(:action pickup
  :parameters (?ob)
  :precondition (and (clear ?ob) (on-table ?ob) (arm-empty))
  :effect (and (holding ?ob) (not (clear ?ob)) (not (on-table ?ob)) 
               (not (arm-empty))))
